New Physics with PeV Astrophysical Neutrino Beams

Astrophysical neutrinos allow us to access energies and baselines that cannot be reached by human-made accelerators, offering unique probes of new physics phenomena. This thesis aims to address the challenges currently facing searches for Beyond Standard Model (BSM) physics in the high-energy universe using astrophysical neutrinos, particularly in the contexts of flavor measurements and connections with dark matter.

==> chapters/taurunner/examples/const_slab.tex <==
The user may use the \texttt{radial} track to propagate neutrinos from a `slab' of material of a constant density.
This may be done by making a \texttt{Body} object on the fly in the following manner.

\begin{lstlisting}[language=python, caption={\textbf{\textit{Propagation of $\nu_{\mu}$ through a constant slab.}} Although \taurunner{} only supports spherical bodies, we may use a body of constant density along with a \texttt{radial} trajectory to propagate a particle through a slab of constant density. One may create the slab from the base $Body$ object or use the \texttt{body.slab} object. We do the former here for pedagogical purposes, but we recommend using the latter in practice since it has some computational speed ups.}]
import numpy as np

from taurunner.body import Body
from taurunner.main import run_MC
from taurunner.cross_sections import CrossSections
from taurunner.utils import make_propagator, make_initial_e, make_initial_thetas

nevents  = 5000
eini     = 1e15
theta    = 0
pid      = 14
xs_model = "CSMS"

# Make body with density 3.14 g/cm^3 and radius 1000 km
body     = Body(3.14, 1e3)

xs       = CrossSections(xs_model)
energies = make_initial_e(nevents, eini)
thetas   = make_initial_thetas(nevents, theta)

tau_prop = make_propagator(pid, body)
rand     = np.random.RandomState(seed=7)

output   = run_MC(energies, 
                  thetas, 
                  body, 
                  xs, 
                  tau_prop, 
                  rand,
                  flavor=pid
)
\end{lstlisting}

==> chapters/taurunner/examples/custom_flix.tex <==
The user may also input custom spectra to sample from.
These should be given to \taurunner{} as pickled splines of the flux's cumulative density function.
An example on how to construct these splines in the appropriate format is given in \ref{app:cdf_energy}.
The default \taurunner{} distribution includes splines of different GZK models.
In this example, we show how to sample energies according to the flux predicted in \cite{ahlers:2010fw}.

\begin{lstlisting}[language=python, caption={\textbf{\textit{Propagating a flux drawn from a provided cumulative distribution function (CDF).}} Example of propagating $\nu_{\tau}$ with energies drawn from a user-provided flux. TauRunner provides a few CDFs for the user, or custom CDFs may be built.}]
import numpy as np

import taurunner as tr
from taurunner.main import run_MC
from taurunner.body.earth import construct_earth
from taurunner.cross_sections import CrossSections
from taurunner.utils import make_propagator, make_initial_e, make_initial_thetas

nevents  = 5000
pid      = 16
xs_model = "CSMS"

Earth    = construct_earth(layers=[(4., 1.0)])
xs       = CrossSections(xs_model)

tau_prop = make_propagator(pid, Earth)
rand     = np.random.RandomState(seed=7)

# Sample from pickled CDF
pkl_f    = f'{tr.__path__[0]}/resources/ahlers2010_test.pkl' # Path to pickle file with CDF to sample from
energies = make_initial_e(nevents,
                          pkl_f, 
                          rand=rand
)
                         
# Sample uniform in solid angle over hemisphere   
th_min = 0 # Minimum nadir angle to sample from
th_max = 90 # Maximum nadir angle to sample from  
thetas = make_initial_thetas(nevents, 
                             (th_min, th_max), 
                             rand=rand
)

output = run_MC(energies, 
                thetas, 
                Earth, 
                xs, 
                tau_prop, 
                rand
)
\end{lstlisting}

This may also be accomplished using the command line interface by running:

\begin{lstlisting}[language=bash]
python main.py -n 1000 -e ./resources/ahlers2010_cdf_spline.pkl -t range --th_min 0 --th_max 90 -s 7 --xs CSMS

\end{lstlisting}

==> chapters/taurunner/examples/installation.tex <==
\taurunner{} can be installed using \texttt{pip3} by running:

\begin{lstlisting}[language=bash]
pip3 install taurunner
\end{lstlisting}

This will also install any required dependencies, which include \texttt{numpy}~\cite{vanderWalt:2011bqk}, \texttt{scipy}~\cite{Virtanen:2019joe}, and \texttt{PROPOSAL}~\cite{Koehne:2013gpa}.

Furthermore, certain use cases may require access to the source code, which can be downloaded from the \taurunner{} \href{https://github.com/icecube/TauRunner}{GitHub}. After obtaining the source code, one can install the source code with the package manager \texttt{pip3}, while allowing the user to make edits to the source code without having to reinstall the package.

\begin{lstlisting}[language=bash, caption={\textbf{\textit{Installing \taurunner{} using \texttt{pip3} with access to source files}}}]
CLONE_DIR=/path/to/clone/directory
cd $CLONE_DIR
git clone https://github.com/icecube/TauRunner.git && cd TauRunner
pip3 install -e .
\end{lstlisting}


Alternatively, for those that do not use the \texttt{pip3} package manager, one can install all of the dependencies listed in the \texttt{requirements.txt} file included on GitHub, and then clone the repository and add the base directory to the \texttt{PYTHONPATH} variable, as follows:

\begin{lstlisting}[language=bash, caption={\textbf{\textit{Installing \taurunner{} from source.}}}]
CLONE_DIR=/path/to/clone/directory
cd $CLONE_DIR
git clone https://github.com/icecube/TauRunner.git
export PYTHONPATH=$PYTHONPATH:$CLONE_DIR/TauRunner
\end{lstlisting}

==> chapters/taurunner/examples/layered_slab.tex <==
The constant density slab may be generalized to a slab of multiple layers.
As mentioned in Sec.~\ref{subsec:track}, the densities in each layer may be positive scalars, unary functions which return positive scalars, or a potentially mixed list of such objects.
In this example, we show how to accomplish this latter option.

\begin{lstlisting}[language=python, caption={\textbf{\textit{Propagation of $\nu_{\tau}$ through a layered slab.}} We may employ the same strategy of using a \texttt{radial} trajectory to replicate propagation through a slab to propagate through a slab with varying properties.}]
import numpy as np

from taurunner.body import Body
from taurunner.main import run_MC
from taurunner.cross_sections import CrossSections
from taurunner.utils import make_propagator, make_initial_e, make_initial_thetas

nevents  = 1000
eini     = 1e15
theta    = 0
pid      = 16
xs_model = "CSMS"

# Make layered body with radius 1,000 km
def density_f(x):
    return x**-2/4
densities  = [4, density_f, 1, 0.4]
boundaries = [0.25, 0.3, 0.5, 1] # Right hand boundaries of the layers last boundary should always be 1
body = Body([(d, b) for d, b in zip(densities, boundaries)], 1e3)

xs       = CrossSections(xs_model)
energies = make_initial_e(nevents, eini)
thetas   = make_initial_thetas(nevents, theta)

tau_prop = make_propagator(pid, body)
rand     = np.random.RandomState(seed=7)

output = run_MC(energies, 
                thetas, 
                body, 
                xs, 
                tau_prop, 
                rand
)
\end{lstlisting}

==> chapters/taurunner/examples/monochromatic.tex <==
Here we give an example of how to use the most fundamental functionality of \taurunner{}: propagating a monochromatic flux of neutrinos at a fixed energy through a body at a fixed angle.

\begin{lstlisting}[language=Python, caption={\textbf{\textit{Propagating a monochromatic flux from a single angle.}} Example of using an independent script to propagate a monochromatic flux of neutrinos with initial energy $E_{\nu}=10^{10}~{\rm{GeV}}$ from a nadir angle of $89^{\circ}$, \textit{i.e.} one degree below the horizon.}]
import numpy as np

from taurunner.main import run_MC
from taurunner.body.earth import construct_earth
from taurunner.cross_sections import CrossSections
from taurunner.utils import make_propagator, make_initial_e, make_initial_thetas

nevents  = 5000 # number of events to simulate
eini     = 1e19 # initial energy in GeV
theta    = 89.0 # incidence angle (nadir)
pid      = 16 # PDG MC Encoding particle ID (nutau)
xs_model = "CSMS" # neutrino cross section model 

Earth    = construct_earth(layers=[(4., 1.0)]) # Make Earth object with 4km water layer
xs       = CrossSections(xs_model)
energies = make_initial_e(nevents, eini) # Return array of initial energies in eV
thetas   = make_initial_thetas(nevents, theta)

tau_prop = make_propagator(pid, Earth)
rand     = np.random.RandomState(seed=7)

output = run_MC(energies, 
                thetas, 
                Earth, 
                xs,
                tau_prop, 
                rand,
         )
\end{lstlisting}

If you are using the source code installation, you may also achieve this same effect from the command line in the following manner

\begin{lstlisting}[language=bash]
python main.py -n 1000 -e 1e19 -t 89 --xs CSMS -s 7 --save /path/to/outdir/output.npy
\end{lstlisting}

The \texttt{--save} flag tells the program where to save the output.
If this is not specified, the output will be printed as a table.

==> chapters/taurunner/examples/power_law.tex <==
\taurunner{} also allows the user to sample initial neutrino energies from a power law distribution.
For this, the user must provide bounds on the minimum and maximum allowed energies.
Furthermore, the user may sample incidence angles to simulate a isotropic flux.
We demonstrate bot of these features in the following example.

\begin{lstlisting}[language=Python, caption={\textbf{\textit{Multiangle injection with energies drawn from a powerlaw distribution.}} Example of propagating a flux of neutrinos with initial energies sampled from a power law with incidence angles uniformly sampled over a hemisphere.}]
import numpy as np

from taurunner.main import run_MC
from taurunner.body.earth import construct_earth
from taurunner.cross_sections import CrossSections
from taurunner.utils import make_propagator, make_initial_e, make_initial_thetas

nevents        = 5000 # number of events to simulate  
pid            = 16
xs_model       = "CSMS"
no_secondaries = True

Earth = construct_earth(layers=[(4., 1.0)])
xs    = CrossSections(xs_model)
rand  = np.random.RandomState(seed=7)

# Sample power-law with index -2 between 1e6 GeV and 1e12 GeV
pl_exp   = -2 # power law exponent
e_min    = 1e15 # Minimum energy to sample in eV
e_max    = 1e21 # Maximum energy to sample in eV
energies = make_initial_e(nevents,
                          pl_exp, 
                          e_min=e_max, 
                          e_max=e_min, 
                          rand=rand
                         )
                         
# Sample uniform in solid angle over hemisphere
th_min = 0 # Minimum nadir angle to sample from
th_max = 90 # Maximum nadir angle to sample from
thetas = make_initial_thetas(nevents, 
                             (th_min, th_max), 
                             rand=rand
                            )

# tracks   = make_tracks(thetas)
tau_prop = make_propagator(pid, Earth)


output = run_MC(energies, 
                thetas, 
                Earth, 
                xs, 
                tau_prop, 
                rand,
                no_secondaries=no_secondaries
               )
\end{lstlisting}

This may also be accomplished via the command line interface by running:

\begin{lstlisting}[language=bash]
python main.py -n 1000 -e -2 --e_min 1e15 --e_max 1e21 -t range --th_min 0 --th_max 90 -s 7 --xs CSMS

\end{lstlisting}

==> chapters/taurunner/examples/radial.tex <==
Besides the chord trajectory, which simulates neutrinos passing through a body from one side to the other, \taurunner{} provides a radial trajectory, which simulates neutrinos originating from the center of a \Body{}.
To use this, one need only modify the call to the \texttt{make\_tracks} function.
Note that the \texttt{theta} argument which was specified previously has no bearing on this, but must be passed due to implementation issues.

\begin{lstlisting}[language=python, caption={\textbf{\textit{Example of propagating $\nu_{\tau}$ along a radial trajectory.}} TauRunner allows for arbitrary particle trajectories. This example shows how to use the \texttt{radial} trajectory, whereas all previous examples have used the \texttt{chord} trajectory.}]
import numpy as np

from taurunner.main import run_MC
from taurunner.body.earth import construct_earth
from taurunner.cross_sections import CrossSections
from taurunner.utils import make_propagator, make_initial_e

nevents  = 5000
eini     = 1e19
pid      = 16
xs_model = "CSMS"

Earth    = construct_earth(layers=[(4., 1.0)]) # Make Earth object with 4km water layer
xs       = CrossSections(xs_model)
energies = make_initial_e(nevents, eini)
thetas   = np.zeros(nevents)

tau_prop = make_propagator(pid, Earth)
rand     = np.random.RandomState(seed=7)

output = run_MC(energies, 
                thetas,
                Earth, 
                xs, 
                tau_prop, 
                rand,
)
\end{lstlisting}

This can also be accomplished from the command line by running:

\begin{lstlisting}[language=bash]
python main.py -n 1000 -e 1e19 -t 89 --xs CSMS -s 7 --track radial
\end{lstlisting}

==> chapters/taurunner/examples/sun.tex <==
In addition to the Earth, \taurunner{} allows for propagation in the Sun.
\taurunner{} includes high- and low-metalicity Suns, and a user may provide their own solar model.
We include an example of the form that these solar models should take in Appendix~\ref{app:solar_model}.

\begin{lstlisting}[language=python, caption={\textbf{\textit{Propagating $\nu_{\tau}$ through the Sun.}} Example of how to propagate $\nu_{\tau}$ through a body besides earth.}]
import numpy as np
from taurunner.main import run_MC
from taurunner.body import construct_sun
from taurunner.cross_sections import CrossSections
from taurunner.utils import make_propagator, make_initial_e, make_initial_thetas, units

nevents     = 5000
eini        = 1e13 # the sun is opaque at high energies
theta       = 10.0
pid         = 16
xs_model    = "dipole"
solar_model = "HZ_Sun" # Can also be "LZ_Sun"
                                   
xs       = CrossSections(xs_model)
energies = make_initial_e(nevents, eini)
thetas   = make_initial_thetas(nevents, theta)

sun      = construct_sun(solar_model)
tau_prop = make_propagator(pid, sun, granularity=0.5) 
rand     = np.random.RandomState(seed=7)

output = run_MC(energies, 
                thetas, 
                sun, 
                xs, 
                tau_prop, 
                rand
)
\end{lstlisting}

The same result may be achieved from the command line by running;

\begin{lstlisting}[language=bash]
python main.py -n 1000 -e 2.4e17 -t 45 -s 7 --body HZ_Sun --xs dipole
\end{lstlisting}
